Kernelizing Temporal Exploration Problems

We study the kernelization of exploration problems on temporal graphs. A temporal graph consists of a finite sequence of snapshot graphs $\mathcal{G}=(G_1, G_2, \dots, G_L)$ that share a common vertex set but might have different edge sets. The non-strict temporal exploration problem (NS-TEXP for short) introduced by Erlebach and Spooner, asks if a single agent can visit all vertices of a given temporal graph where the edges traversed by the agent are present in non-strict monotonous time steps, i.e., the agent can move along the edges of a snapshot graph with infinite speed. The exploration must at the latest be completed in the last snapshot graph. The optimization variant of this problem is the $k$-arb NS-TEXP problem, where the agent's task is to visit at least $k$ vertices of the temporal graph. We show that under standard computational complexity assumptions, neither of the problems NS-TEXP nor $k$-arb NS-TEXP allow for polynomial kernels in the standard parameters: number of vertices $n$, lifetime $L$, number of vertices to visit $k$, and maximal number of connected components per time step $\gamma$; as well as in the combined parameters $L+k$, $L + \gamma$, and $k+\gamma$. On the way to establishing these lower bounds, we answer a couple of questions left open by Erlebach and Spooner. We also initiate the study of structural kernelization by identifying a new parameter of a temporal graph $p(\mathcal{G}) = \sum_{i=1}^{L} (|E(G_i)|) - |V(G)| +1$. Informally, this parameter measures how dynamic the temporal graph is. Our main algorithmic result is the construction of a polynomial (in $p(\mathcal{G})$) kernel for the more general Weighted $k$-arb NS-TEXP problem, where weights are assigned to the vertices and the task is to find a temporal walk of weight at least $k$.

==> old-kernel.tex <==
We have seen so far, that there is no polynomial kernel for \textsc{NS-TEXP} in the parameter $n$. Another approach for a parameter leading to a polynomial kernel is to bound the dynamic behavior of the graph in terms of edge appearances. Observe that in order to visit all vertices, we need to cross at least $n-1$ edges. Hence, a temporal graph with less than $n-1$ appearances of an edge in total is a trivial no-instance. This gives us a lower-bound of $n-1$ edge appearance which allows us to consider the above-guarantee parameter $p = \mathfrak{m} - n$ where $\mathfrak{m}$ is the total number of edge appearances. More formally, if $\mathcal{G} = (G_1, G_2, \dots, G_L)$ is the input temporal graph, then $\mathfrak{m} = \sum_{i=1}^{L} |E(G_i)|$.


\begin{theorem}
	\label{thm:kernel-p}
	\textsc{NS-TEMP} admits a polynomial kernel of size $\mathcal{O}(TODO)$ in the above-guarantee parameter $p = \mathfrak{m}-n$.
\end{theorem}
\todo[inline,color=magenta]{Write proof sketch for the kernel?}
\begin{proof}
Let $\mathcal{G} = (G_1, G_2, \dots, G_L)$ be the input temporal graph.
The parameter $p$ bounds the number of edges of $\mathcal{G}$ that appear more than once during the lifetime. From now on, we will call edges that appear only once \emph{blue edge} and edges appearing more than once \emph{red edges}. We will also assume that $G$ is connected as otherwise $\mathcal{G}$ is a trivial no-instance.

We begin with some observation for the case that blue edges form bridges in the underlying graph $G$ of $\mathcal{G}$.
Assume the blue edge $e$ is a bridge between some components $C_1$ and $C_2$ in $G$. Let $t$ be the unique time step in which $e$ is present. Then, if one of the components $C_1$ and $C_2$ is connected in time step $t$, then we can remove this component. To prove this, assume without loss of generality that $C_1$ is connected in time step $t$. As $e$ appears only once, we can split any temporal exploration into two phases. We start in one of the components and are only able to cross to the other component in time step $t$. Assume we start our temporal exploration in $C_2$. Now, if in time step $t$, all vertices of $C_1$ are connected and the bridge $e$ is present, we can visit in this time step all vertices of $C_1$ and end our move in this time step on the endpoint of $e$ that lays in $C_2$. In other words, we do not need to properly \emph{cross} the bridge and wait on some vertex in $C_1$ in order to visit all vertices in $C_1$. Hence, we can collapse the component $C_1$ to a single vertex. In the case that the temporal exploration started in $C_1$, by the arguments above we can find a temporal exploration starting in the vertex in $C_2$ that is incident to $e$.
This leads us to our first reduction rule:

\textbf{Reduction rule 1:} Let $e$ be a bridge consisting of a blue edge in $G$. Let $t$ be the unique time step in which $e$ is present. Then, collapse every component containing an endpoint of $e$ that is connected in time step $t$.


\begin{claim}
	\label{claim:forbidden}
	After applying reduction rule~1 exhaustively on a graph~$G$, either,  $G$ is a no-instance, or $G$ does not contain a structure as depicted in \autoref{fig:forbidden} consisting of three blue bridges that do not lay on a single path where the components $C_1$, $C_3$, and $C_4$ contain more than one vertex.
\end{claim}
We assume in the following that we applied reduction rule~1 exhaustively.
\begin{claimproof}
	Assume we applied reduction rule~1 exhaustively on $G$ but $G$ still contains the forbidden structure afterwards. Then, each of the components $C_1$  $C_3$, and $C_4$ contains more than one vertex. 
	By the assumption, that we applied reduction rule~1 exhaustively, the component $C_1$ is not connected in the time step in which $e_{12}$ is present.
	Further, $C_3$ is not connected in the time step in which $e_{23}$ is present and $C_4$ is not connected in the time step in which $e_{24}$ is present. As each of the edges $e_{12}$, $e_{23}$, and $e_{24}$ is only present in one time step, we cannot cross any of them twice in two different time step. 
	Now assume we have a temporal exploration scheme that starts in some component $C_1$, $C_3$, $C_4$. Without loss of generality, assume, we start in some vertex in $C_1$. Then, at some time, we needs to visit some vertex in $C_2$. From there, we can only reach any vertex in $C_3$ by crossing the edge $e_{23}$ in the unique time-step $t_{23}$ in which $e_{23}$ is present. Respectively, we can only reach any vertex in $C_4$ by crossing the edge $e_{24}$ in the unique time-step $t_{24}$ in which $e_{24}$ is present. Now assume $t_{12} \leq t_{23} \leq t_{24}$. As $C_3$ is not connected in time-step $t_{23}$, in order to visit all vertices of $C_3$, we need to end the time step $t_{23}$ on some vertex in $C_3$ and thereby `properly' cross the edge $e_{23}$. But now, we can no longer visit all vertices in $C_4$ as we cannot reach $C_2$ from $C_3$ at any time-step $t > t_{23}$. This yields a contradiction to the assumption that we have a temporal exploration scheme for $G$. It is easy to see that we obtain a similar contradiction if we assume that the temporal exploration starts in $C_2$.
\end{claimproof}
\begin{figure}
	\centering
	\begin{tikzpicture}
	\node at (0,0) {$C_1$};
	\draw (0,0) ellipse (1cm and 0.7cm);
	
	\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (1) at (1,0) {};
	\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (2) at (2,0) {};
	
	\node at (3,0) {$C_2$};
	\draw (3,0) ellipse (1cm and 0.7cm);
	
	\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (3) at (3.85,0.35) {};
	\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (4) at (5,1) {};
	
	\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (5) at (3.85,-0.35) {};
	\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (6) at (5,-1) {};
	
	\node at (6,1) {$C_3$};
	\draw (6,1) ellipse (1cm and 0.7cm);
	\node at (6,-1) {$C_4$};
	\draw (6,-1) ellipse (1cm and 0.7cm);
	
	\path[thick,draw=blue]
	(1) edge node[above] {$e_{12}$} (2)
	(3) edge node[above left] {$e_{23}$} (4)
	(5) edge node[below left] {$e_{24}$} (6)
	;
	\end{tikzpicture}
\caption{text}
\label{fig:forbidden}
\end{figure}

%Now, assume $C_1$ and $C_2$ are not connected in time step $t$. Let $\operatorname{end}_1$ be the earliest time step, in which a temporal exploration can visit all vertices in $C_1$ and let $\operatorname{start}_1$ be the latest time step in which a temporal exploration must start in order to still visit all vertices in $C_1$. Respectively, define $\operatorname{end}_2$ and $\operatorname{start}_2$ analogously for $C_2$. Then, if $\operatorname{end}_1 > t$ and $\operatorname{end}_2 > t$ it is clear that $\mathcal{G}$ is a no-instance, as we are forced to change between $C_1$ and $C_2$ in time step $t$ and are not able to visit all vertices of one of the components before this time step. As we are not able to cross the edge $e$ again to come back to a component, we cannot reach all vertices. The same holds if  $\operatorname{start}_1 < t$ and $\operatorname{start}_2 < t$. Further, if $\operatorname{end}_1 < t < \operatorname{end}_2$ it is clear that any temporal exploration must start in $C_1$. The same holds if $\operatorname{start}_1 < t < \operatorname{start}_2$. Analogous conditions can be derived for starting in $C_2$.

We are now ready to consider the structure in $G$ induced by the blue and red edges. Let $X$ be the set of endpoints of red edges in $G$.
Now, observe that our parameter $p = \mathfrak{m}-n$ bounds the size of a minimum \emph{feedback edge set} for $G$. Further, we can find such a minimum feedback edge set in polynomial time~\cite{todo}\todo{ref}.
Assume we have found a minimum feedback edge set for $G$.
Now, we can add to $X$ all endpoints of edges in the feedback edge set. The set $X$ is now of size TODO\todo{todo}.
If we remove from $G$ the set of edges having both endpoints in $X$ (denote this by $G\setminus E(X)$), we obtain a forest consisting only of blue edges. At this point, some of those trees can have multiple leaves in $X$ as depicted in \autoref{fig:kernel-prestep}. We will deal with this case next.
\begin{figure}
	\centering
	\begin{tikzpicture}
		\draw (0,0) ellipse (6cm and 0.5cm);
		\node at (0,0) {$X$};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (1) at (-2,0.3) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (2) at (-2,1) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (3) at (-1,1.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (4) at (0,2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (5) at (1,1.8) {};		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (6) at (2,1) {};		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (7) at (2,0.3) {};
		\path[] 
		(1) edge (2)
		(2) edge (3)
		(3) edge (4)
		(4) edge (5)
		(5) edge (6)
		(6) edge (7);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (8) at (1.6,2.1) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (9) at (1.7,1.8) {};
		
		\path
		(5) edge (8)
		(5) edge (9);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (10) at (2.5,1.3) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (11) at (2.5,0.7) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (12) at (3,1.6) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (13) at (3,1) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (14) at (3.5,1.3) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (15) at (3.5,0.7) {};
		
		\path
		(6) edge (10)
		(6) edge (11)
		(10) edge (12)
		(10) edge (13)
		(13) edge (14)
		(13) edge (15);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (16) at (-1.5,1.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (17) at (-2,2.1) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (18) at (-2,1.5) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (19) at (-2.5,1.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (20) at (-2.5,1.2) {};
		
		\path
		(3) edge (16)
		(16) edge (17)
		(16) edge (18)
		(18) edge (19)
		(18) edge (20);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (21) at (-4.5,0.2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (22) at (-4,0.2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (23) at (-3.5,0.2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (24) at (-3,0.2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (25) at (-4.25,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (26) at (-3.25,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (27) at (-3.75,1.5) {};
		
		\path
		(25) edge (21)
		(25) edge (22)
		(26) edge (23)
		(26) edge (24)
		(27) edge (25)
		(27) edge (26);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (28) at (6,1.5) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (29) at (5.5,1.5) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (30) at (5,1.5) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (31) at (4.5,1.5) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (32) at (5.75,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (33) at (4.75,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (34) at (5.25,0) {};
		
		\path
		(28) edge (32)
		(29) edge (32)
		(30) edge (33)
		(31) edge (33)
		(32) edge (34)
		(33) edge (34);
	\end{tikzpicture}
%	\includegraphics[width=5cm]{kernel-prestep.png}
	\caption{text}
	\label{fig:kernel-prestep}
\end{figure}

Therefore, we want to find a set $S$ of vertices in $V(G)\setminus X$ that we add to $X$ in order to get rid of trees outside of $X$ having multiple leaves in $X$. We begin with setting $S = V(G)\setminus X$. Now, recursively remove from $S$ all vertices of degree one in $G(S \cup N(S))$, i.e., the neighborhood closure of $S$. When we do not find any next vertex of degree one to remove, we are left with some trees in $G \setminus E(X)$ having \emph{all} their leaves in $X$.
We now add all vertices in $S$ of degree at least three to the set $X$. Therefore, we show that the number of vertices of degree at least three in $S$ is bounded by $|X|^2$.

Therefore, observe that:
\begin{claim}
	\label{claim:noshare}
	No two trees in $G(S\cup N(S))$ can share more than one leaf in $X$. 
\end{claim}
\begin{claimproof}
	Assume this is not the case and two trees in $G(S\cup N(S))$ share at least two leaves in $X$. But then, we find a cycle in $G\setminus E(X)$ which contradicts that $X$ contains all endpoints of the edges in a feedback edge set.
\end{claimproof}
Now we can find an upper bound on the number of trees in $G(S\cup N(S))$ where no two trees share more than one leaf in $X$. 
Note that trees with only one leaf in $X$ have already be removed from $S \cup N(S)$. Therefore, we only need to count the number of trees with at least two leaves in $X$.
Fix some vertex $v$ in $X$ that will be a maximally shared leaf. Then, we get the maximal number of trees with at least two leafs in $X$ sharing only the vertex $v$ as a leaf if each tree has exactly two leafs. As there are $|X|-1$ possibilities for the second (not shared) leaf, we obtain $|X|-1$ many trees that can share the vertex $v$. As there are $|X|$ possible choices for the shared vertex $v$, the claimed upper bound follows.


%Now we want to ensure\todo[color=magenta]{Why?} that the vertices in $X$ are only leaves or roots of the trees outside of $X$, i.e., no tree grows through some vertex in $X$. Therefore, observe that the number of vertices $v\in V\setminus X$ that have at least three neighbors in $X$ is bounded by the size of $X$\todo{Why?}.

At this point, $X$ contains all endpoints of red edges, all end points of edges in a feedback edge set, and all vertices of degree at least three in the set $S$. Hence, the graph $G \setminus E(X)$ now contains only trees with roots in $X$ and trees with at most one leaf (and possibly the root) in $X$. 
%Now, $G\setminus E(X)$ can be depicted as in \autoref{fig:kernel-modulator}.
Recall that in a tree, every edge is a bridge.
We now give some more arguments about trees consisting of blue edges. 
%More precisely, we show that:
\begin{claim}
	\label{claim:caterpillar}
	After applying reduction rule~1 exhaustively on a tree $T$ consisting of blue edges, the tree is a either a caterpillar or we can output no. 
\end{claim}
\begin{claimproof}
	The claim follows directly by observing that any tree on blue edges that is not a caterpillar contains the forbidden structure depicted in~\autoref{fig:forbidden}. Hence, by \autoref*{claim:forbidden} we can identify such a tree as a no-instance.
%Assume we applied reduction rule~1 exhaustively on $T$ but $T$ is not a caterpillar afterwards. Then, $T$ contains the graph $H$ depicted in \autoref{fig:subgraph} as an induced subgraph where vertex 1 is considered to be the root. 
%By the assumption, that we applied reduction rule 1 exhaustively, it holds that there exists an edge in the subtree routed at vertex 6 that appears at a different time step than the edge $(3,6)$. The same holds for the subtree rooted at vertex 4 with respect to the edge $(3,4)$. By the same assumption we find an edge to the left of vertex 2 that appears at a different time step than the edge $(2,3)$. As we can cross a blue edge at most once and have to properly wait a time step in the subtrees rooted at the vertices 4, 6, and in the subtree to the left of vertex 2\todo[color=magenta]{how to call this tree?} we cannot visit all vertices on $T$.
\end{claimproof}
\begin{figure}
	\centering
	\begin{tikzpicture}
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (1) at (0,0) {1};
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (2) at (1.5,0) {2};
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (3) at (3,0) {3};
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (4) at (4.5,-0.5) {4};
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (5) at (6,-0.5) {5};
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (6) at (4.5,0.5) {6};
		\node[circle,draw=black,inner sep=0pt,minimum size=10pt] (7) at (6,0.5) {7};
		\path[thick] 
		(1) edge (2)
		(2) edge (3)
		(3) edge (4)
		(4) edge (5)
		(3) edge (6)
		(6) edge (7);
	\end{tikzpicture}
	\caption{text}
	\label{fig:subgraph}
\end{figure}

Now, we can assume that $G\setminus E(X)$ only consists of caterpillars where only the endpoints may be contained in $X$. The graph $G\setminus E(X)$ can now be depicted as in \autoref{fig:kernel-modulator}.
\begin{figure}
	\centering
	\begin{tikzpicture}
		\draw (0,0) ellipse (6cm and 0.5cm);
		\node at (0,0) {$X$};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (1) at (-2,0.3) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (2) at (-2,1) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (3) at (-1,1.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (4) at (0,2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (5) at (1,1.8) {};		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (6) at (2,1) {};		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (7) at (2,0.3) {};
		\path[] 
		(1) edge (2)
		(2) edge (3)
		(3) edge (4)
		(4) edge (5)
		(5) edge (6)
		(6) edge (7);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (8) at (1.6,2.1) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (9) at (1.7,1.8) {};
		
		\path
		(5) edge (8)
		(5) edge (9);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (10) at (2.5,1.3) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (11) at (2.5,0.7) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (12) at (-2,1.6) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (13) at (-2.4,1.4) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (14) at (3.5,1.3) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (15) at (3.5,0.7) {};
		
		\path
		(6) edge (10)
		(6) edge (11)
		(2) edge (12)
		(2) edge (13);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (16) at (-1.5,2) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (17) at (-2,2.1) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (18) at (-2,1.5) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (19) at (-2.5,1.8) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (20) at (-2.5,1.2) {};
		
		\path
		(3) edge (16);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (21) at (-4,0.2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (22) at (-4.8,0.6) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (23) at (-4.5,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (24) at (-4.2,0.9) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (25) at (-3.9,0.9) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (26) at (-3.6,0.78) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (27) at (-3.3,0.6) {};
		
		\path
		(21) edge (22)
		(21) edge (23)
		(21) edge (24)
		(21) edge (25)
		(21) edge (26)
		(21) edge (27);
		
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (28) at (3.3,2.2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (29) at (3.5,1.7) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (30) at (4,2) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (31) at (4.5,1.5) {};
%		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (32) at (5.75,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (33) at (4.75,0.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (34) at (5.25,0) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (35) at (5.2,1.8) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (36) at (5.2,1.3) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (37) at (5.4,0.7) {};
		\node[circle,draw=black,fill=black,inner sep=0pt,minimum size=5pt] (38) at (4.,0.9) {};
		
		\path
		(28) edge (30)
		(29) edge (30)
		(30) edge (31)
		(31) edge (33)
		(33) edge (34)
		(33) edge (37)
		(33) edge (38)
		(31) edge (35)
		(31) edge (36);
	\end{tikzpicture}
%	\includegraphics[width=5cm]{kernel-modulator.png}
	\caption{text}
	\label{fig:kernel-modulator}
\end{figure}
Next, we show that the number of caterpillars in $G\setminus E(X)$ is bounded by a polynomial in $|X|$ before we conclude with proving that each caterpillar in $G\setminus E(X)$ can be replaced by a caterpillar of constant size.

By similar arguments as for \autoref{claim:noshare}, no two caterpillars in $G\setminus E(X)$ can share two vertices in $X$ as we would otherwise obtain a cycle in contradiction to $X$ containing a feedback edge set. Hence, the number of caterpillars in $G\setminus E(X)$ with two endpoints in $X$ can be bounded by $|X|^2$.
Now, consider caterpillars in $G\setminus E(X)$ with only one vertex in $X$. As we assume that we applied reduction rule~1 exhaustively, there can only be two non-trivial caterpillars (consisting of more than one vertex) with one endpoint in $X$ as we would otherwise obtain the forbidden structure in~\autoref{fig:forbidden}. 

What remains is a potentially unbounded number of trivial caterpillars, or in other words, stars of arbitrary degree with center in $X$. We now show that we can replace any star consisting only of blue edges by a star with at most $p+|X|^2 +1$\todo{this bound can be improved} many rays. 

\textbf{Reduction rule 2:} Let $v\in X$ be a center of a star with (only) blue edges to the pendent vertices $u_1, u_2, \dots, u_\ell$ with $\ell > p+|X|^2+1$. Recall, that $|X|$ is polynomial in $p$. Without loss of generality assume that $t_1, t_2, \dots, t_\ell$ are the unique time steps in which the edges $e_{v{u_1}}, e_{v{u_2}}, \dots, e_{v{u_\ell}}$ are present such that $t_1 \leq t_2 \leq \dots \leq t_\ell$. The number of edge appearances in $E(X)$ is bounded by $p+|X|^2$. Mark each time step in which some edge in $E(X)$ appears in the lifetime of $\mathcal{G}$. Now, if $v$ has more than $p+|X|^2$ many pendant vertices, then at least two consecutive time steps $t_i$ and $t_{i+1}$ must lay between two marked time steps. As the corresponding vertices $u_i$ and $u_{i+1}$ are of degree one and connected only with a blue edge, any temporal exploration schedule must visit the vertex $v$ in time step $t_i$ and in time step $t_{i+1}$. As both time steps are between two marked time steps with respect to edge appearances in $X$, the exploration schedule cannot leave $v$ between time-step $t_{i}$ and $t_{i+1}$ as $X$ is an independent set in any time step $t$ with $t_{i} < t < t_{i+1}$. Hence, for each sequence $t_{i}, t_{i+1}, \dots, t_{j}$ that lays between two marked time-steps with respect to the edge appearances in $X$, we can delete the vertices $u_{i+1}, \dots, u_{j}$ and only keep $u_i$.
Now we have that also the number of trivial caterpillars in $G\setminus E(X)$ is bounded by a polynomial in our parameter.

We conclude by showing that each non-trivial caterpillar in $G\setminus E(X)$ can be replaced by a path of length at most three. 
Recall that each caterpillar in $G\setminus E(X)$ only consists of blue edges. Further, each edge in the backbone of the caterpillar is a bridge. 
Fix some non-trivial caterpillar and let $v_0, v_1, \dots, v_\ell$ be the vertices of the backbone of the caterpillar. Let $t_1, t_2, \dots t_\ell$ be the time-steps in which the edges $e_{01}, e_{12}, \dots, e_{(\ell-1) \ell}$ of the backbone are present. Further, for $1 \leq i < \ell$, let $t_{i,1}, t_{i,2}, \dots t_{i,{k_i}}$ be the time-steps in which the pendent edges of $v_i$ are present.
Without loss of generality, assume $t_{i,1} \leq t_{i,2} \leq \dots \leq t_{i,{k_i}}$. 


\todo[inline,color=magenta]{Define caterpillar, backbone, leg and assume that it starts and end in a backbone vertex. Define $E(X)$.}

\textbf{Reduction rule 3:} Consider the the case that the considered caterpillar is one of the two non-trivial caterpillars with one endpoint in $X$. As we cannot cross blue edges twice, it is clear that any exploration schedule must start in the endpoint not contained in $X$ of one of them and end in the endpoint not contained in $X$ of the other.  
Assume we picked the caterpillar in which the exploration starts, as the other case is analogous.
Further, assume that $v_0$ is not in $X$. Then, it must hold (i) that $t_i \leq t_{i,1} \leq t_{i,{k_i}} \leq t_{i+1}$ for $1 \leq i \leq \ell-1$ as otherwise, we would need to cross a blue edge twice. Thereby, the traversal through the caterpillar is fixed, and any exploration scheme will leave $v_0$ in time step $t_1$, traverses along the backbone and leaves the caterpillar over the edge $e_{(\ell-1)\ell}$ in time step $t_\ell$. Hence, we can  replace the caterpillar satisfying condition (i) by a path of length two consisting of the vertices $v_0$, $v_1$, and $v_\ell$ with an edge between $v_0$ and $v_1$ that is only present in time step $t_{1}$ and an edge between $v_1$ and $v_\ell$ that is only present in time step $t_\ell$.

\textbf{Reduction rule 4:} Consider a non-trivial caterpillar with both endpoints in $X$. As there might be a path between $v_0$ and $v_\ell$ in $X$ it might be possible to avoid crossing over the backbone of the caterpillar and instead visit some part of the caterpillar in time step $t_1$ over the vertex $v_0$ and the remaining part over the vertex $v_\ell$ in time step $t_\ell$. Hence, we can have the following three cases where we refer to the first case in the order that applies as the case at hand.\todo[color=magenta]{don't know how to say this, see it as an if (else if) else}
\begin{enumerate}
	\item There exists $1 \leq j \leq \ell$ such that $t_i = t_j$ for all $i\leq j$ and $t_{j+2} = t_{i'}$ for all $i'$ with $j+2 \leq i' \leq \ell$
	\item $t_i \leq t_{i,1} \leq t_{i,{k_i}} \leq t_{i+1}$ for $1 \leq i \leq \ell-1$
	\item The first two cases do not apply. 
\end{enumerate}
Assume the first case holds. Then, we can replace the caterpillar by a path of length three consisting of the vertices $v_0$, $v_j$, $v_{j+1}$, $v_\ell$ with an edge between $v_0$ and $v_j$ that is only present in time-step $t_j$, an edge between $v_j$ and $v_{j+1}$ that is only present in time-step $t_{j+1}$, and an edge between $v_{j+1}$ and $v_\ell$ that is only present in time-step $t_\ell$. \todo[color=magenta]{Do I need to say anything about correctness? I find it pretty obvious}

Now assume that the first case does not hold but the second case holds. Then, there exists some vertices $v_{j'}$ and $v_{j''}$ such that $t_{j'} \leq t_{j''}$ and further $t_1 < t_{j'}$ and $t_{j''} < t_\ell$ as otherwise the first case would have hold. Now, continue with replacing the caterpillar by a path of length three as in the first case by giving $t_{j'}$ the role of $t_j$ and $t_{j''}$ the role of $t_{j+1}$.

Now assume that neither the first, nor the second case applies. 
Then, there exist time-steps $t_j$, $t_{j'}$, and $t_{j''}$ such that $t_j \leq t_{j''}$, $t_{j'} < t_j$ and $t_{j''} < t_j$. Now, remove the edge between $v_{j'-1}$ and $v_{j'}$, and apply reduction rule~1, 2, and 3 again exhaustively. If, afterwards, we are left with more than two non-trivial caterpillars with exactly one endpoint in $X$, output no, otherwise, continue with an other caterpillar with two endpoints in $X$.


\todo[inline,color=magenta]{Should we rewrite some of the checks for being a no-instance as explicit reduction rules?}

Now, after applying reduction rules 1 to 4 exhaustively, we are left with a set $X$ of size TODO\todo{todo} and a polynomial number of constant-sized caterpillars outside of $X$. This concludes the construction of our polynomial kernel for \textsc{NS-TEXP} of size TODO\todo{todo}.

\end{proof}

